Neural Sign Actors: A diffusion model for 3D sign language production from text

Sign Languages (SL) serve as the primary mode of communication for the Deaf and Hard of Hearing communities. Deep learning methods for SL recognition and translation have achieved promising results. However, Sign Language Production (SLP) poses a challenge as the generated motions must be realistic and have precise semantic meaning. Most SLP methods rely on 2D data, which hinders their realism. In this work, a diffusion-based SLP model is trained on a curated large-scale dataset of 4D signing avatars and their corresponding text transcripts. The proposed method can generate dynamic sequences of 3D avatars from an unconstrained domain of discourse using a diffusion process formed on a novel and anatomically informed graph neural network defined on the SMPL-X body skeleton. Through quantitative and qualitative experiments, we show that the proposed method considerably outperforms previous methods of SLP. This work makes an important step towards realistic neural sign avatars, bridging the communication gap between Deaf and hearing communities.

==> Tables/backtranslation.tex <==
\begin{table}[!h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccc}
    \toprule
    \textbf{Method} & \textbf{BLEU-4} & \textbf{BLEU-3} & \textbf{BLEU-2} & \textbf{BLEU-1}  & \textbf{ROUGE}  
    \\
    \midrule 
        ProgressiveTransformer \cite{saunders2020progressive} &  &  & &  & \\
        Stoll \etal \cite{stoll2018sign}  &  &  & & &\\

        \textbf{Proposed}  & & & & &\\
    \bottomrule
    \end{tabular}}
    \caption{Quantitative evaluation of the proposed and the baseline methods on How2Sign test dataset. }
    \label{tab:backtranslation}
\end{table}


==> sec/acknowledgements.tex <==
\noindent\textbf{Acknowledgements.}SZ was supported by EPSRC Project DEFORM (EP/S010203/1) and GNOMON (EP/X011364). RP was supported by EPSRC Project GNOMON (EP/X011364).
